Leveraging Hierarchical Taxonomies in Prompt-based Continual Learning

Humans perceive the world as a series of sequential events, which can be hierarchically organized with different levels of abstraction based on conceptual knowledge. Drawing inspiration from human learning behaviors, this work proposes a novel approach to mitigate catastrophic forgetting in Prompt-based Continual Learning models by exploiting the relationships between continuously emerging class data. We find that applying human habits of organizing and connecting information can serve as an efficient strategy when training deep learning models. Specifically, by building a hierarchical tree structure based on the expanding set of labels, we gain fresh insights into the data, identifying groups of similar classes could easily cause confusion. Additionally, we delve deeper into the hidden connections between classes by exploring the original pretrained model's behavior through an optimal transport-based approach. From these insights, we propose a novel regularization loss function that encourages models to focus more on challenging knowledge areas, thereby enhancing overall performance. Experimentally, our method demonstrated significant superiority over the most robust state-of-the-art models on various benchmarks.

==> arvix/A_sec/0-abstract.tex <==
Drawing inspiration from human learning behaviors, this work proposes a novel approach to mitigate catastrophic forgetting in Prompt-based Continual Learning models by exploiting the relationships between continuously emerging class data. 
We find that applying human habits of organizing and connecting information can serve as an efficient strategy when training deep learning models. Specifically, by building a hierarchical tree structure based on the expanding set of labels, we gain fresh insights into the data, identifying groups of similar classes could easily cause confusion.
Additionally, we delve deeper into the hidden connections between classes by exploring the original pretrained model's behavior through an optimal transport-based approach. From these insights, we propose a novel regularization loss function that encourages models to focus more on challenging knowledge areas,  thereby enhancing overall performance. Experimentally, our method demonstrated significant superiority over the most robust state-of-the-art models on various benchmarks. 
% Our code is available at \url{https://anonymous.4open.science/r/HierC-089B/}.

% % Firstly, we uncover that the forgetting phenomenon in PCL models mainly occurs due to the introduction of new classes that may overlap with the old ones in the latent space. To address this, the model must effectively distinguish between old and new data, especially those with many similar characteristics. 



==> arvix/A_sec/1-intro.tex <==
% {\color{blue} Nhat: References?}
Continual Learning (CL) \citep{wang2024comprehensivesurveycontinuallearning, DBLP:conf/nips/Lopez-PazR17} is a research direction focused on realizing the human dream of creating truly intelligent systems, where machines can learn on the fly, accumulate knowledge, and operate in constantly changing environments as a human's companion. Despite the impressive capabilities of A.I systems, continual learning remains a challenging scenario due to the tendency to forget obtained knowledge when facing new ones, known as \textit{catastrophic forgetting} \citep{french1999catastrophic}. In dealing with this challenge, traditional CL methods often rely on storing past data for replaying during new tasks, which can raise concerns about memory usage and privacy. To overcome this limitation, recent methods proposed leveraging the generalizability of pre-trained models \citep{han2021pre, jia2022visual} as frozen backbones to solve sequences of CL tasks \citep{wang2022dualprompt, smith2022coda, li2024steering}.
% achieving state-of-the-art performance on various continual learning benchmarks.


% P1: Human learning ---> CL ----> Traditional CL's drawback... privacy, require taskID when inference, forgetting.. .catastrophically.. --> Pretrained Continual Learning... 





While these pre-trained-based methods have demonstrably achieved impressive results, only consider forgetting caused by changes in learned prompts or differences between the (prompt-based) models chosen for training and testing \citep{wang2023hierarchical, tran2023koppa, cprompt}. Further completing those arguments, we show that forgetting of old knowledge also comes from the uncontrolled growth of new classes in the latent space. That is, models are confused in distinguishing between old and new classes, which many methods overlook when training tasks independently \citep{smith2022coda, wang2022learning_l2p}.
Furthermore, we find that current approaches only utilize limited information from the training dataset and treat class labels equally during training, resulting in missing opportunities to further enhance model representations and mitigate forgetting more effectively.


In addition, we find that human natural learning behavior has many valuable aspects, especially the habit of analyzing data, organizing them in a meaningful way, and finding connections between old and new knowledge \citep{schon1983reflective, bransford2000how, sweller1988cognitive, mayer2005cambridge}, thereby improving the ability to understand, remember, and reproduce information. 
Inspired by this, we investigate the characteristics of current common benchmark datasets as well as the behavior of pre-trained-based CL models, showing that the incoming data classes over time can always be categorized into consistent groups.
Each such group usually includes class data with similar semantic characteristics, which is easy to get confused by models and should be paid special attention to during training.  

Therefore, we propose a training strategy that constantly considers emerging data in groups, following a hierarchical tree-like taxonomy developed based on expert/domain knowledge. During training new tasks, the model references information from old classes in the tree. Especially, the feature extractor is encouraged to maximally contrast and distinguish concepts/labels within the same group, also promoting the learning of common features that can be transferred to new concepts/labels in the same group in future tasks. This strategy not only mitigates forgetting when new classes emerge but also consolidates domain-specific knowledge. Besides, by considering human learning habits, we also find that individuals with better foundations will absorb knowledge faster and more effectively. Thus, we propose an optimal-transport-based technique to further exploit prior knowledge from pretrained models, where the behavior of this starting model will reveal a new view of the relationships between classes. Moreover, we propose a testing strategy where the characteristics of each group aid in identifying data samples, especially those located at the boundaries between different leaf groups of the taxonomy.

% further exploit prior knowledge from pretrained models, where the behavior of this starting model
% will reveal a new view of the relationships between classes. Moreover, we propose a testing strategy where the characteristics of each group aid in identifying data samples, especially those located at
% the boundaries between different leaf groups of the taxonomy.
% Furthermore, we observe that images belonging to concepts/labels within the same group in the hierarchical taxonomy share strong visual and semantic correlations, leading to overlapping representations in the latent space, which compromises performance. By encouraging the feature extractor to separate and contrast the representations of images in these concepts/labels more distinctly, we effectively reduce the overlap of easily confused classes, thereby improving performance. 
% Additionally, to further exploit the hierarchical taxonomy, we propose a testing strategy that leverages the group's characteristics to better identify data samples, especially those near boundaries between different groups in the taxonomy. 

% Therefore, we propose a training strategy that constantly considers emerging data in groups, following a hierarchical tree-like taxonomy. In particular, during learning new tasks, a model always
% references information from old classes in the tree. Especially, the data in the same group will
% be applied a specific constraint to encourage the model to deeply understand the detailed knowledge contained in that group. This strategy not only helps the model avoid forgetting when new
% classes appear, but also consolidates the model’s knowledge in specific domains corresponding to
% each group. By considering human learning habits, we also find that individuals with better foundations will absorb knowledge faster and more effectively. Thus, we propose a novel technique to
% further exploit prior knowledge from pretrained models, where the behavior of this starting model
% will reveal a new view of the relationships between classes. Moreover, we propose a testing strategy where the characteristics of each group aid in identifying data samples, especially those located at
% the boundaries between different leaf groups of the taxonomy.


\textbf{Contribution.} We name our method as \emph{Leveraging Hierarchical \textbf{T}axonomies in Prompt-based \textbf{C}ontinual \textbf{L}earning} (TCL), and summarize our main contributions as follows:

\begin{itemize}
    \item We introduce a new perspective to explain the reason for catastrophic forgetting in pretrained-based Continual learning models, which potentially comes from the uncontrolled growth of incoming classes on the latent space.
    
    \item Originating from the research findings of Cognitive Science, we propose a novel approach to reduce forgetting by exploiting relationships between data. By dynamically building label-based hierarchical taxonomies and leveraging the initial behavior of the pretrained model, we can identify the challenging knowledge areas that further focus, and determine how to learn them during the sequence of tasks. Based on this taxonomical structure, our testing strategy further improves model performance.
    


    
    % where classes with similar characteristics are consistently grouped.
    % In addition, to further extract the hidden connection between different classes of data, we offer another strategy ... 
    % Additionally, our testing strategy leveraging cluster information helped improve the model's prediction probability.
    
    \item We empirically evaluate the effectiveness of our method against current state-of-the-art pre-trained-based baselines across various benchmarks.
    
\end{itemize}

\textbf{Organization.} The rest of the paper is structured as follows. In Section \ref{relatedW}, we present related work. Then in Section \ref{background}, we formulate the problem and introduce a new perspective to explain the cause of forgetting in CL models. Section \ref{method} transitions from the motivation provided by Cognitive Science insights to the proposed training and testing strategy, emphasizing the importance of exploiting relationships between class data. Section \ref{exp} presents the experimental results, and finally, we discuss the limitations and suggest future directions in Section \ref{conclusion}.

% In summary, our contributions... 
% ------------------------------------

% - Inspired by human behavior when learning new things, dive deep + connect with old stuffs 


% ---> Training: detail, find connection between information that has been learned and is being learned via manipulating latent space....

% + Take advantage of the prior (base) knowledge from pretrained model...

% ----> testing:Exploiting the relationships of learned information during inference + prior from base model...


% \subsection{Motivations}



% * CIFAR:
% HIDE:  92.61
% + tt (92.81)

% Ours: 93.98
% train only: 93.52 


% -------------------------\\
% * ImgNetR:
% HiDe: 75.06 
% + tt (75.22)

% Ours: 76.41
% train_only: 76.02

% -------------------------\\
% * CUB: 
% HiDE: 86.62
%  + tt (86.75)

% Ours: 88.02
% train_only: 87.80



==> arvix/A_sec/2-1-relatedW.tex <==
% \textbf{Continual Learning.} Continual learning \citep{ DBLP:conf/nips/Lopez-PazR17, masana2022class, le2024mixtureexpertsmeetspromptbased} tackles the challenge of incrementally training a model on a sequence of tasks, while mitigating the risk of 
% The main problem of Continual Learning is finding the way to mitigate \textit{catastrophic forgetting} \citep{mccloskey1989catastrophic, nguyen2019toward}, where previously learned knowledge is lost as new tasks are introduced. 
\paragraph{Class Incremental Learning.}
This is one of the most challenging and widely studied CL scenarios \citep{van2019three, wang2023hierarchical}, where task identity is unknown during testing, and data of previous data is inaccessible during current training \citep{DBLP:journals/pami/MasanaLTMBW23, DBLP:conf/cvpr/RebuffiKSL17, DBLP:conf/cvpr/HouPLWL19, pmlr-v162-guo22g}.
% Most successful CIL methods rely on storing and rehearsing old training data, which introduces concerns around efficiency and privacy \citep{rebuffi2017icarl, wang2021memory, cha2021co2l}. Recently, approaches leveraging the strong generalization abilities of pre-trained models have emerged, achieving state-of-the-art performance on various benchmark datasets \citep{zhou2023revisiting, wang2023isolation, mcdonnell2023ranpac}. 
This work follows the setting of CIL and proposes a novel approach to mitigate forgetting and improve performance for prompt-based CL models.
% , which take advantage of pretrained models as frozen backbones.  


% \vspace{-2mm}
\paragraph{Prompt-based Continual Learning.}
This line of work exploits the power of pre-trained backbone to quickly adapt to the sequence of downstream tasks by updating just a small number of parameters (prompts).
Initial work like \cite{wang2022learning_l2p, wang2022dualprompt, smith2022coda} typically assign a set of prompts to tasks, enhancing the adaptability of the backbone to downstream tasks. However, the absence of explicit constraints can lead to feature overlapping between classes from different tasks. Therefore, recent methods employ some types of contrastive loss \citep{wang2023hierarchical, li2023steering} or utilize Vision Language models \citep{DBLP:conf/nips/WangHH22, DBLP:conf/wacv/NicolasCZADD24} to better separate features from tasks.
However, they treat all classes equally during training, missing the opportunity to learn in challenging areas where classes have many similarities and are easily confused. In this work, we propose a novel approach to exploit the relationships within data, allowing the model to recognize groups of these classes, and develop a deeper understanding of the respective knowledge areas, thereby reducing forgetting and enhancing its ability to learn new tasks.



==> arvix/A_sec/2-2-background.tex <==
\subsection{Problem formulation and Notations}
% We consider the Continual learning setting in which a model is required to learn from a sequence of classification tasks. Each task $t \in \{1, ..., T\}$ has a training dataset $D_t$ with $n_t$ i.i.d. samples $\{(\boldsymbol{x}_t^i, y_t^i)\}_{i=1}^{n_t}$, and $T$ may be unknown or infinite. The model needs to learn these tasks sequentially, without replaying data from old tasks during training and without access to task ID when inference. 
% This approach is often known as \textit{rehearsal-free Continual Learning} \citep{smith2022coda, wang2023hierarchical}.

We consider the Class Incremental Learning setting \citep{Zhou_2024, lopez2017gradient_gem, wang2023hierarchical}, where a model has to learn from a sequence of $T$ visual classification tasks without revisiting old task data during training or accessing task IDs during inference. Each task $t \in \{ 1, ..., T\}$ has a respective dataset $\mathcal{D}_t$, containing $n_t$ i.i.d. samples ${(\boldsymbol{x}_t^i, y_t^i)}_{i=1}^{n_t}$. Let $D_c = (X_c,  Y_c)$ denote the data corresponding to the class label $c$.

In this work, we design our model as a composition of two components: \textit{a pre-trained ViT backbone} $f_\Phi$ and \textit{a classification head} $h_\psi$. That is, we have the model parameters $\theta = (\Phi, \psi)$. Similar to other existing prompt-based methods, we incorporate into the pre-trained ViT a set of prompts $\bm{P}$. We denote the overall network after incorporating 
the prompts as $f_{\Phi, \bm{P}}$. 

\subsection{Forgetting in Prompt-based Continual Learning} \label{sec:forgetting}
% Typically, CL models face the challenge of forgetting old knowledge when learning new ones (i.e., \textit{catastrophic forgetting}). Over time, 

In CL models, changes in the dataset, including inputs $\bm{X}$ in the input space $\mathcal{X}$ and labels $\bm{Y}$ in the label space, $\mathcal{Y}$ lead to the changes of model's behavior \textit{(feature shift)} and thus model's performance on previously learned tasks to decrease significantly (i.e., \textit{catastrophic forgetting}).
% For networks trained from scratch, this phenomenon occurs due to changes in parameters $\theta$, which alter the model's behavior, leading to uncontrollable shifts in features $f_{\theta}(\bm{X})$ corresponding to data from old tasks (see Table \ref{tab:compareCL}). 
% Additionally, the limitation in accessing old task data causes the model's knowledge about these tasks to diminish gradually.
% \begin{table}[ht]
%     \centering
%     \begin{tabular}{lll}
%     \hline
%          & Conventional CL & Prompt-based CL \\
%          \hline
%          \hline 
%          Input space $\mathcal{X}$ & \multicolumn{2}{c}{$p(X_t) \neq p(X_{t+1})$} \\
%          Label space $\mathcal{Y}$ & \multicolumn{2}{c}{$Y_t \cap Y_{t+1} =  \varnothing $} \\
%          \hline 
%          Parameter space $\Theta$ & $\theta^*_t \neq \theta^*_{t+1}$ & $\theta^*_t = \theta^*_{t+1}$ \footnote{We consider prompt-based models where each task $t$ is dedicated to a separate set of prompts $\bm{P}_t$, which then is fixed after training.}\\
%          Latent space $\mathcal{Z}$ & $f_{\theta^*_t} (X) \neq f_{\theta^*_{t+1}}(X)$ & $f_{\widehat{\theta}_t} (X) \approx f_{\widehat{\theta}_{t+1}}(X)$ \\
%          \hline
%     \end{tabular}
%     \caption{Comparison between two main approaches for CIL setting, where $\theta^*_t$ is parameters of model optimized for $(\bm{X}_t, \bm{Y}_t)$ after learning task $t$, $\hat{\theta }_t$ is the selected parameters (prompted model) when testing for prompt-based CL.}
%     \label{tab:compareCL}
% \end{table}
Current prompt-based CL methods, which leverage the power of pretrained models, attribute forgetting/feature shift either to \textbf{(I)} changes in parameters from the backbone when using the common prompt pool $\bm{P}$ for all tasks \citep{wang2022learning_l2p, wang2022dualprompt} or to \textbf{(II)} the inherent mismatch between the models used at training and testing. Specifically, let $\hat{t}(\bm{x})$ and $t(\bm{x})$ as the chosen promptID and the ground-truth promptID for $\bm{x}$, respectively. We may have  
$f_{\hat{\theta}_t} = f_{\Phi, \bm{P}_{\hat{t}}} \neq f_{{\theta}_t} = f_{\Phi, \bm{P}_{{t}}}
$ because there are chances that the promptID $\hat{t} \neq t$, where $\hat{t}$ is predicted by pretrained backbone $f_\Phi$ (Figure \ref{fig:promptID}), as discussed and analyzed in \cite{cprompt, tran2023koppa}.
To complement these views, below we provide an empirical study to offer new insights about the reason for forgetting in this type of model, which arises from overlapping between old and new class representations. 
% {\color{blue}Tuan: we can summarize our conclusions here, what are those insights? "Our investigations suggest/show/conclude that...", as far as I understand, it's about the overlapping phenomena of new classes. Also, should we say something at the beginning of Section 4 to connect with the message of this Section? The two sections are a bit disconnected for now.}

Firstly, to completely eliminate concerns about changing learned parameters, we consider methods that propose using a distinct set of prompts $\bm{P}_t$ to a specific task $t$. Then, the remaining potential factor of \textit{forgetting by feature shift} is the difference between the prompt chosen at inference time and the one used during training (i.e., $\bm{P}_t \neq \bm{P}_{\hat{t}}$).
% {\color{blue} Tuan: Maybe move the definitions of $t$ and $\hat{t}$ to the previous paragraph, at the sentence "the inherent mismatch between..."}. 
Thus, we conduct experiments on HiDE \citep{wang2023hierarchical} (i.e., the latest SOTA in prompt-based CL) to measure the differences between the features formed when using these two prompts.  
Particularly, we consider $\bm{x} \in D_1$ that belongs to the first task and measure the L2 Wasserstein distance $W_2(Q, \hat{Q})$ \citep{kantorovich1939mathematical} between $Q$ (i.e., the latent distribution corresponding to $\bm{P}_t$, which consists of  $f_{\Phi, \bm{P}_{{t}(\bm{x})}}(\bm{x})$ for $\bm{x} \sim D_1$) and $\hat{Q}$ (i.e., the latent distribution corresponding $\bm{P}_{\hat{t}}$ after learning the last task, consists of $f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x})$ for for $\bm{x} \sim D_1$). 
% More specifically, $\hat{Q}$ consists of feature vectors $f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x})$ for $\bm{x} \sim D_1$, while $Q$ consists of $f_{\Phi, \bm{P}_{t(\bm{x})}}(\bm{x})$ for for $\bm{x} \sim D_1$. 
% {\color{blue} TUan: How do we measure the distribution shift in Table \ref{tab:shift}, is it the Wasserstein distance? If it is $W_2(Q, \hat{Q})$, maybe we should include the explicit formula of $W_2(Q, \hat{Q})$, I'm not really sure if it's needed.} 
The results in Table \ref{tab:shift} show that the difference of these distributions is apparently negligible in many cases when using pretrained backbone Sup-21K. 

\begin{figure}[htbp]
    \centering
    % First row: Figure A and Table B
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/promptID_accuracy.pdf} % Replace with your image file
        \caption{PromptID accuracy}
        \label{fig:promptID}
    \end{subfigure}
    % \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \vspace{-9mm}
        \centering
        \resizebox{.7\textwidth}{!}{
        \begin{tabular}{lc}
            \toprule
              & Sup21K  \\
            \midrule
            Split-Imagenet-R & $3.23\times10^{-6}$  \\
            Split-CIFAR100 & $2.46\times 10^{-6}$  \\
            Split-CUB-200 & $2.15\times10^{-6}$  \\
            \bottomrule
        \end{tabular}}
        \captionof{table}{\small Distribution
        shift.}
        \vspace{8mm}
        % \caption{Distribution shift}
        \label{tab:shift}
    \end{minipage}

    \vspace{0.5em} % Space between rows

    % Second row: Figure C, D, and E
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        % height=35.45mm
        \includegraphics[width=\textwidth, height=42.1mm]{img/within_task_accuracy.pdf} % Replace with your image file
        \caption{Within task accuracy on $D_1$}
        \label{fig:wt_a}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{img/true_accuracy.pdf} % Replace with your image file
        \caption{True accuracy on $D_1$}
        \label{fig:true_a}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/overal_accuracy.pdf} % Replace with your image file
        \caption{Overall accuracy}
        \label{fig:overal_a}
    \end{subfigure}

    \caption{\textbf{Empirical study about forgetting (HiDE).} \textbf{(a)} Average accuracy of promptID prediction for all tasks; \textbf{(b)} Accuracy of the first task over time, using classification head $s_1$ (Sup-21K); \textbf{(c)} Accuracy of the first task over time, using classification head $h_\psi$ (Sup-21K); \textbf{(d)} Average accuracy on all tasks so far, after learning each task (Sup-21K).\textbf{ Table \ref{tab:shift}} (Distribution shift) reports L2 Wasserstein distance between the latent distributions corresponding to $\bm{P}_t$ and $\bm{P}_{\hat{t}}$ of data task 1, after learning the final task.}
\label{fig:insight}
\vspace{-3mm}
\end{figure}

For a closer look, besides \textit{the main classification head} $h_\psi$ used for all classes so far, at the end of each task $t$, we set up \textit{a specific classifier} $s_t$ optimized on the frozen latent space of $D_t$ and then kept fixed. From now on, we refer to the accuracy measured on $D_t$ using \( s_t \) as \textit{'within task accuracy'}, and the accuracy using \( h_\psi \) as \textit{'true accuracy'} of this task. The results in Figure \ref{fig:wt_a}, show that \textit{within task accuracy} of the first task stays almost unchanged, which concurs with our observation on the negligible shift between $f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x})$ and $f_{\Phi, \bm{P}_{t(\bm{x})}}(\bm{x})$.
% Furthermore, in Figure \ref{fig:true_a}, we measure the \textit{true performance} of the task (i.e., the accuracy when using the classification head for all classes so far over the features \( f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x}) \)) over time. 
Meanwhile, we observe a significant decrease in the corresponding \textit{true performance} in Figure $\ref{fig:true_a}$, raising the question of whether we have overlooked additional factors contributing to final forgetfulness (Figure \ref{fig:overal_a}), beyond the issue of selecting incorrect task prompts during inference.


% ???? 
% To identify the cause of the performance degradation despite the negligible shift, we now investigate the \textit{inference feature space} of \( f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x}) \). 
% Although there is a minor shift between \( f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x}) \) and \( f_{\Phi, \bm{P}_{t(\bm{x})}}(\bm{x}) \), leading to good performance if the correct classification head is chosen, as more tasks arrive, the number of classes and classification heads increases. This results in greater overlap in the \textit{inference feature space}, causing more confusion for the classification heads when making predictions. 

Considering the \textit{inference feature space} of \( f_{\Phi, \bm{P}_{\hat{t}(\bm{x})}}(\bm{x}) \), we can see that as more tasks arrive, the number of classes increase, making the space fuller and increasing the possibility of overlap between class distributions.
% To further demonstrate the increasing overlap and filling of the inference feature space, 
To demonstrate this point, we provide t-SNE visualization of class representations in 
Figure \ref{fig:tnse} and the respective illustration in Figure \ref{fig:train}. In particular, after Task 1, we have representations of "oak tree", "mouse" and "porcupine" located in quite separate locations. However, when Task 2 and then Task 3 arrive, the appearance of "willow tree" and "pine tree" makes the latent space become fuller, and "oak tree" no longer maintains the separation from the remaining classes as before and even its representation may even be misassigned to other classes, leading to a remarkable drop in performance.  

% Experimentally, Table \ref{tab:shift} shows that this change of features from Task 1 on latent space measured by Wasserstein distance: \textcolor{red}{$\Delta = W(f_{\Phi, \bm{P}_{\hat{t}}}(D_1), f_{\Phi, \bm{P}_{{t}}} (D_1))$} apparently negligible in many cases, and the \textit{within task accuracy} of the first task is almost unchanged (Figure \ref{fig:wt_a}). Despite this, the \textit{true performance} of that task decreases over time (Figure \ref{fig:true_a}), raising the question of whether we have overlooked any other factors that cause final forgetfulness \ref{fig:overal_a}.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{meomeo.pdf}
%     \caption{\textbf{[TABLE/ FIGURE A - insights about the performance and latent space of each task over time] - running, HIDE, CODA (Sup21, Dino) - taskID accuracy, within task accuracy, true accuracy, shift-WSD]}}
%     \label{fig:insight}
% \end{figure}

% Without loss of generality, consider the backbone to be frozen and unchanging over time.
% % Looking closer at the latent space of $f_{\Phi, \bm{P}_{\hat{t}}}$, 
% Looking closer at the respective latent space, assume that after learning task 1, the latent space contains representations of classes $c^1_1$ and $c^1_2$. The probability of a data sample $\bm{x}$ predicted belonging to its ground truth label $y_{\bm{x}} = c^1_1$ is: 
% \begin{equation}
%     p(c^1_1|\bm{x}) =  1 -  p(c^1_2|\bm{x}) = a^1_1
% \end{equation}
% After learning task $2$, suppose we have features a new class $c^{2}_1$ on the latent space. Therefore,  
% \begin{equation}
%     p(c^1_1|\bm{x}) =  1 -  \left[p(c^1_2|\bm{x}) + p(c^2_1|\bm{x}) \right] \leq a^1_1
% \end{equation}

% That is, a model can feasibly lose its ability on a certain task when learning new ones, even when the related knowledge is still stored safely in the model (in the form of fixed prompts, with the corresponding features in the latent space remaining unchanged). In particular, the value of \( p(c^1_1|\bm{x}) \) will decrease whenever new class \( c' \) appears such that \( d(\bm{x}, c_1^1) > d(\bm{x}, c') \), where the predicted class is the class with the smallest distance from $\bm{x}$. This mainly occurs due to uncontrolled overlap between the features of the old and new tasks.

% Consequently, we can consider another main cause of Catastrophic forgetting in Prompt-based CL is now the addition of new classes, which are distributed in positions that may overlap with the existing locations of the old ones. This appearance leads to confusion in distinguishing classes and making final judgments, thereby reducing performance over time. 
Therefore, another key cause of catastrophic forgetting in prompt-based continual learning (CL) that should be recognized is \textit{the addition of new classes, which gradually fills the latent space and overlaps with existing ones}. This overlap causes confusion in distinguishing between classes, thus reducing performance over time. While existing CL methods emphasize the importance of representation learning to keep classes distinct, none explicitly acknowledge the overlap between new and old tasks as a source of forgetting. 
Recognizing this motivates us to propose a novel method, focusing on identifying easily confused class pairs, thereby reducing forgetting and improving performance.


==> arvix/A_sec/3-framework.tex <==
In the previous section, we noted that increased overlap in data representations as more tasks arrive is one of the main reasons for greater confusion in predictions, leading to performance degradation. It is crucial to identify easily confused classes/concepts to effectively enhance their distinguishability. Inspired by cognitive science studies \citep{schon1983reflective, bransford2000how, mayer2005cambridge}, showing that organizing concepts in a tree-like taxonomy of visually and semantically related items aids memory and retrieval, we propose using expert/domain knowledge to structure the concepts/labels of continual learning (CL) tasks in a hierarchical taxonomy. Interestingly, we find that concepts/labels within the same group in this taxonomy tend to be visually and semantically similar, potentially causing more overlap in the latent space and confusion for the CL classifier. Motivated by this observation, we propose group-based contrastive learning to maximize the distinguishability of these concepts/labels.    

\subsection{Motivation}
% \paragraph{{Insights from Cognitive Science.}} Research has shown that humans better understand and remember information when it is organized or connected meaningfully \citep{bruner1956thinking, sweller1988cognitive, miller1956magical, rogers1977}. One approach that enhances memory retention is associative learning—the idea that information is easier to recall when linked with related concepts or prior knowledge. This type of learning involves strengthening the connections between neurons when they are activated together, a principle known as \textit{Hebbian learning}. Additionally, \textit{elaborative encoding} has been identified as a key technique for improving memory. Studies, such as those by \cite{rogers1977}, have found that when individuals process information in a more meaningful way, such as relating it to themselves or to familiar concepts, they are more likely to remember it. This method leverages the self-reference effect, where personalizing information during learning enhances recall.

\paragraph{Insights from Cognitive Science.} Research in Cognitive Science highlights the importance of \emph{reflection, organization, and linking information} as critical components of effective learning. Studies show that when learners take time to reflect on their experiences, they deepen their understanding and enhance retention \citep{schon1983reflective}. This reflective practice encourages individuals to connect new information with existing knowledge, fostering a more integrated learning experience \citep{bransford2000how}. Moreover, organizing information into coherent structures, such as outlines or concept maps, allows learners to see relationships between concepts, making it easier to retrieve information later \citep{mayer2005cambridge}. Linking new material with relevant prior knowledge—often referred to as associative learning—further strengthens memory retention \citep{sweller1988cognitive} and also benefits future learning.

% Together, these strategies create a robust framework for learning, emphasizing that how information is processed and connected can significantly impact cognitive outcomes.

\paragraph{Our Approach.} It is evident that besides \emph{reflection}, comparison of old and new information, the key factor in learning efficiently is \emph{to organize and exploit them in an insightful way}, where concepts are linked and arranged according to their semantic meanings. This observation motivates us to develop a deep learning classifier that learns labels or concepts structured in a hierarchical taxonomy. The aim is to enable the classifier to grasp relevant concepts more effectively, helping to mitigate the challenge of catastrophic forgetting. More specifically, we propose structuring the data labels in a hierarchical taxonomy, which can be dynamically constructed using domain expertise, adapting as needed based on the specific context and evolving understanding of the domain. Based on this structure, we establish a reference framework for the relationships between classes, identifying which classes belong to the same group with many shared characteristics, easily confused due to overlap, and require more focus (see Figures \ref{fig:motivation_taxonomy}, \ref{fig:tnse}). This approach not only helps the model better avoid forgetting, but also reinforces knowledge to facilitate future learning.

\vspace{-3mm}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{img/hierC_cifar100.pdf}
    % \includegraphics[width=\textwidth]{img/hierC.jpg}
    \vspace{-5mm}
    \caption{The hierarchical taxonomy obtained when learning Task 3 on Split-CIFAR100.}
    \label{fig:motivation_taxonomy}
\end{figure}


\begin{figure}[htbp]
    \centering
    % Subfigure 1
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        % height=5.551cm
        \includegraphics[width=\textwidth, height=6.568cm]{img/tSNE_coda.pdf} % Replace with your image file
        \caption{Training tasks independently with $\mathcal{L}_{CE}$}
        \label{fig:L_CE}
    \end{subfigure}
    \hfill % Adds horizontal space between the subfigures
    % Subfigure 2
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/tSNE_hide.pdf} % Replace with your image file
        \caption{Ours (HiT)}
        \label{fig:L_G}
    \end{subfigure}
    \caption{t-SNE visualization of classes within leaf groups of Four-legged animals ($ \bullet $ circular points) and Plants ($\blacktriangle$ triangular points) when learning Task 3, Split-CIFAR100.}
    \label{fig:tnse}
\end{figure}

Taking the learning process of Split-CIFAR100 as an example, when training on task \( t=3 \), we can construct a tree-like taxonomy of concepts/labels, as shown in Figure \ref{fig:motivation_taxonomy}. We observe that the concepts/classes under the same leaf in the tree-like taxonomy (e.g., oak tree, willow tree, and pine tree in the "plants" leaf group) exhibit stronger visual and semantic correlations. Consequently, as shown in Figure \ref{fig:tnse}a, their features in the feature space become more overlapping compared to those from other leaf groups (e.g., otter and hamster under the "four-legged" leaf group), leading to more confusion and performance degradation when predicting these concepts/classes. This highlights the impact of organizing concepts/labels in a tree-like taxonomy, where data examples within the same leaf group share stronger visual and semantic relationships, causing greater overlap and increased confusion during predictions. Linking to our analysis in Section \ref{sec:forgetting}, the tree-like taxonomy of concepts/labels serves as a tool to help identify easily confused classes/concepts, facilitating the subsequent process of making them more distinct and separable in the feature space. 


Our approach aims to train the backbone network so that all class representations must be distinct, especially those within each leaf group, to achieve maximum distinguishability.
For the leaf group of four-legged animals, we assume that "mouse" and "porcupine" arrive in Task 1, while "otter" and "hamster" are in Task 3.  When learning Task 1, to classify "mouse" and "porcupine", the backbone is encouraged to capture the essential features of four-legged mammals to efficiently differentiate between these two animals. We hope that the knowledge learned from "mouse" and "otter" in Task 1 can be beneficial for the next tasks. Then in Task 3, we again learn to distinguish "hamster", "otter" and these old ones in this group. In this way, the mechanism helps further strengthen the learning of more efficient and robust features for the Mammals group.

To summarize, by grouping and categorizing, we expect the model to concentrate more on the detailed features of each leaf group. This enhances its ability to distinguish related objects and reinforces the model's knowledge of each group. Therefore, this strategy not only alleviates the forgetting of old knowledge—often caused by new classes that are difficult to distinguish from old ones within the same leaf group, but also enables active knowledge transfer between tasks.


\subsection{Training phase}
\subsubsection{Exploiting hierarchical label/concept taxonomy}

% \textbf{[Figure of method - how to develop the taxonomy over time, and how we strengthen knowledge about each group...]}

\begin{wrapfigure}{r}{0.55\textwidth}
    \centering
    \vspace{-13mm}
    \includegraphics[width=0.55\textwidth]{img/train.pdf}
    \vspace{-8.8mm}
    \caption{We focus on separate easily confused classes within each leaf group.}
    \label{fig:train}
\end{wrapfigure}

During the training process, whenever a new class appears, its label name is automatically added to the tree-like taxonomy, into a leaf group containing classes with similar characteristics (Figure \ref{fig:motivation_taxonomy}). To develop this hierarchical structure, we can rely on expert knowledge, for example, ChatGPT, which can help us incrementally construct a meaningful and semantically-related tree (see Appendix \ref{chatGPT}). Structuring information in this way not only aligns with how the human brain effectively connects and remembers information but also provides useful insights during training, indicating how each knowledge is related to the other and which requires further focus.


As analyzed above, reflecting on and organizing knowledge is the key factor for efficient learning. That is, the model should always be encouraged to identify the decision boundary between all old and new classes, especially those in the same leaf group. 
Assume that we finished the task $t-1$ and are learning the prompt $\bm{P}_t$ for task $t$, our aim is to learn the backbone network $f_{\Phi, \bm{P}_t}$ that can minimize overlap between all classes so far, especially focus on increasing the separability between classes belonging to the same leaf group extracted from the taxonomy (e.g., four-legged mammals, plants, etc.,). Let $g \in \mathcal{G}$ be a leaf group, ${X}^g_{k}$ and ${Y}^g_{k}$  denote the corresponding sets of input samples and labels under the group $g$ that belong to the task $k$ ($k \leq t$). Besides Cross Entropy loss $\mathcal{L}_{CE}$, we propose using a regularization loss function for sample $\vx$ (arrives in task $t$, belong leaf group $g$) as follows:
\begin{equation}
    \mathcal{L}_\mathcal{G}(\psi, \bm{P}_t, \bm{x}) = - \alpha \log \sum_{\vx'\in X^g_{t}|y_{\vx'}=y_\vx} \frac{u(\vz_x \cdot  \vz_{x'})}{\sum_{\bar{x} \in X^g_{\overline{1,t}}} u(\vz_x \cdot  \vz_{\bar{x}}) 
    } - \beta \mathcal{L}_{all},
    \label{group_loss}
\end{equation}
where $\displaystyle \mathcal{L}_{all} = \log \sum_{\vx'\in X^g_{t}|y_{\vx'}=y_\vx} \frac{u(\vz_x \cdot  \vz_{x'})}{\sum_{\bar{x} \in X_{\overline{1,t}}} u(\vz_x \cdot  \vz_{\bar{x}})
    }$ is the Supervised Contrastive loss that we force all class representations so far to separate from each other, $u(\vz_\vx \cdot  \vz_{\vx'}) = \exp( \frac{\vz_\vx \cdot  \vz_{\vx'}}{\tau})$,
% \begin{equation}
%     \displaystyle  = -\log \sum_{x'\in X_{\overline{1,t}}|y_{x'}=y_x} \frac{ \exp( \frac{\vz_x \cdot  \vz_{x'}}{\tau})}{\sum_{\bar{x} \in X_{\overline{1,t}}} \exp(
%     \frac{\vz_x \cdot  \vz_{x'}}{\tau}
%     ) + \alpha\sum_{g \in \mathcal{G}, \Tilde{x} \in X^g_{\overline{1,t}}} \exp(
%     \frac{\vz_x \cdot \vz_{\Tilde{x}}}{\tau}
%     )}
%     \label{group_loss}
% \end{equation}
with $\vz_\vx = f_{\Phi, \bm{P}_t}(\vx)$ is the feature vector on the latent space of the prompt-based model, $y_\vx$ is the ground truth label of $\vx$, $\tau$ is a temperature ($\tau =0.1$ for all experimental setting), and $\alpha$ is the coefficient that controls how much we want to force on classes belonging to the same leaf group stay apart further.
% \color{red}Tuan: maybe explain the hyperparameter $\alpha$ here, I would say something like "the hyperparameter $\alpha$ controls how much we want to enforce the representation $\vz_x$ to be close to its corresnponding leaf group with the same label"\color{black}. 
For each data sample $\vx | y_\vx \in Y_{k<t}$, the corresponding representation $\vz_\vx$ is sampled from the Gaussian Mixture model $\text{GMM}_{y_\vx} = \{ \mathcal{N}(\mu_{y_\vx}, \Sigma_{y_\vx}) \}_{k=1}^{K}$ of the respective class, which is obtained at the end of each corresponding task. This technique of using pseudo features of old data is also employed in many existing prompt-based CL methods, as the shift of features is minimal (Table \ref{tab:shift}). 

Equation \ref{group_loss} implies that when learning a new task, new classes/new knowledge will be compared and contrasted with existing ones. That is, the model will be encouraged to identify the decision boundary between old and new classes, especially focusing on those in the same leaf group via controllable coefficient $\alpha$ (Figure \ref{fig:train}). 
% This step matches the way our brain naturally works - without reference and comparison, we would be confused about old and new concepts, leading to incorrect judgments and decisions in practice. For AI models, learning new tasks without considering old tasks can lead to uncontrolled overlapping of layer representations in the latent space, resulting in forgetting and harming final performance. 
% Besides, focusing on the specific knowledge in each leaf group also helps our model strengthen and consolidate the understanding about this domain, especially when the current prompt is initialized by the last prompt as we employ the prompt ensemble strategy like in \citep{wang2023hierarchical}: $\bm{P'} = \eta \bm{P}_t + (1-\eta)\sum_{i=1}^{t-1}\bm{P}_i$.
Furthermore, focusing on the specific knowledge within each leaf group helps our model strengthen and consolidate its understanding of this domain, especially when the current prompt is initialized by the previous ones. This is achieved by employing a prompt ensemble strategy similar to that in \citep{wang2023hierarchical}: $\bm{P}_t = \eta \bm{P'}_t + (1-\eta)\sum_{i=1}^{t-1}\bm{P'}_i$, where $\left\{\bm{P'}_i \right\}_{i=1}^t$ is the set of learnable prompt elements which are used to adapt to corresponding tasks, the prompt elements of previous tasks are kept fixed ($\eta = 0.99$ for all setting).

% Consequently, by using the loss function in Equation \ref{group_loss} and finding the appropriate alpha coefficient, the model will enhance its ability to distinguish between data classes, especially those in the same leaf group $g$, which consists of highly similar classes, thereby improving general representation learning and reducing forgetting for CL models.



\subsubsection{An optimal transport-based approach to further exploiting priori from pretrained model}
\label{ot_tricky}

% Although the taxonomy constructed above is a useful information channel that provides a new perspective on the relationship between data, the tree structure is still fundamentally based on the semantic information of the text labels. Condensing information into a few labels is sometimes not enough to describe the myriad characteristics of visual data. 

Considering a leaf group, there may be data classes with varying levels of overlap in the latent space(Figure \ref{fig:tnse}, \ref{fig:ot_trick}). Although focusing on classes within the same leaf group helps improve the ability to recognize difficult-to-identify classes, we still treat all classes in that group equally. Thus, the algorithm may inadvertently ignore important pairs of classes that are easily confused and need to be further distinguished. Besides, pretrained models are known to have been extensively trained on large datasets, resulting in a substantial repository of generalization ability. Therefore, the prior knowledge from these models often provides a valuable starting point for the adaptation to downstream tasks. However, we seem to frequently overlook the initial behavior of pretrained models on the training data, particularly regarding relations between classes, which classes are easily classified and which are prone to confusion. 

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{-5mm}
    % \includegraphics[width=0.55\textwidth]{img/WS_latent_space.pdf}
    \includegraphics[width=0.5\textwidth]{img/WS_latent_space_bblueue.pdf}
    \vspace{-4mm}
    \caption{Wasserterin distance between classes (Split-CIFAR100) in latent space of pre-trained backbone (Sup-21K).}
    % \vspace{-3mm}
    \label{fig:ot_trick}
\end{wrapfigure}

Therefore, in this work, we propose to exploit the pre-trained model from a new perspective, which can comprehend the use of the label-based tree-like taxonomy during training, where we can take advantage of prior assumptions about the relationships between the image classes. Firstly, to extract the relationship between the classes, we use L2 Wasserstein distance (WD) to compare the distributions of feature vectors of each pair of class. In particular, let $D_{c_i}^\Phi$ be the distribution of class $c_i$ on the latent space of the pretrained model $f_\Phi$, which is obtained in the form of a Gaussian Mixture model at the end of the respective task. When $t$ tasks have arrived, we have the corresponding sets of distributions $\{ D_c^\Phi \}_{c \in Y_{1,t}}$ of all $m_t$ classes from all tasks so far. Therefore, we gradually complete the WD-based matrix between pairs of classes:
\begin{equation}
    M= [W_2(D_{c_i}^\Phi, D_{c_j}^\Phi)]_{m_t\times m_t}.
\end{equation}
We then compute \textit{the weight matrix} $\displaystyle \Gamma = \left[ \gamma_{ij}
\right]_{m_t \times m_t} = \left[ 1/ {\exp(M_{ij}/\delta)} \right]_{m_t\times m_t}$, where $\delta$ is a temperature. We then apply this information to obtain a weighted version of $\mathcal{L}_\mathcal{G}$, in which the closer the two class distributions are, the larger the weight assigned, and they will be focused to push away. Consequently, our regularization loss becomes:
\begin{equation}
    \mathcal{L}_\mathcal{G}(\psi, \bm{P}_t, \bm{x}) = - \alpha \log \sum_{\vx'\in X^g_{t}|y_{\vx'}=y_\vx} \frac{u(\vz_x \cdot  \vz_{x'})}{\sum_{\bar{x} \in X^g_{\overline{1,t}}} \gamma_{y_xy_{\Tilde{x}}}u(\vz_x \cdot  \vz_{\bar{x}}) 
    } - \beta \mathcal{L}_{all}.
    \label{group_loss_gamma}
\end{equation} 
% \begin{equation}
%     \mathcal{L}_\mathcal{G}(\theta, P_t, x) = -\log \sum_{x'\in X_{\overline{1,t}}|y_{x'}=y_x} \frac{\exp(\frac{\vz_x \cdot  \vz_{x'}}{\tau})}{\sum_{\bar{x} \in X_{\overline{1,t}}}  \exp(
%     \frac{\vz_x \cdot \vz_{\bar{x}}}{\tau}
%     ) + \alpha\sum_{g \in \gG,\Tilde{x} \in X^g_{\overline{1,t}}} \gamma_{y_xy_{\Tilde{x}}}\exp(
%      \frac{\vz_x \cdot \vz_{\Tilde{x}}}{\tau}
%     )}
%     \label{group_loss_gamma}
% \end{equation}
This strategy is completely economical and aligns well with the CL learning scheme as matric $M$ is continuously expanded and provides useful information for training new tasks. Practically, when learning a new task, the first epoch is spent capturing information about the behavior of the pretrained model on the data for this task. Moreover, this approach is similar to the findings in Cognitive Science \citep{osgood1953communication, baltes1987experience}, showing that the accumulated experiences from past learning create momentum for learning new skills more effectively. 
% Finally, our objective function during training can be formulated as follows ($\beta$ is a hyperparameter): 
% \color{red}
% \begin{equation}
%     \mathcal{L} = \mathcal{L}_{CE} + \beta\mathcal{L_G}
% \end{equation}

% \color{black}

\subsection{Testing phase}

We observe that classes within the same leaf group often share many common characteristics. 
% Leveraging this observation during testing can offer a new perspective to determine the label that a sample $\bm{x}$ belongs to. 
Therefore, we propose a testing strategy that leverages information from each leaf group to gain a new perspective on the identification of data samples, especially those at the boundaries between different leaf groups. 

In particular, the final prediction for sample $\bm{x}$ will be modified based on the probability that $\bm{x}$ belongs to a certain leaf group $g \in \mathcal{G}$ (i.e., $p(g|\bm{x}, \bm{P}_{\hat{t}})$). Intuitively, if the representation $\bm{z}_x$ of $\bm{x}$ has many similarities with class representations in group $g$, then $p(g|\bm{x}, \bm{P}_{\hat{t}})$ will increase, thereby raising the likelihood that $\bm{x}$ belongs to the corresponding classes in $g$ (i.e., $p(y|g, \bm{x},\bm{P}_{\hat{t}})$):
\begin{equation}
    p(y|\bm{x}) = p(y|\bm{x},\bm{P}_{\hat{t}}) = \sum_{g \in \mathcal{G}} p(g|\bm{x},\bm{P}_{\hat{t}}) \cdot p(y|g, \bm{x}, \bm{P}_{\hat{t}}) = \sum_{g \in \mathcal{G}} p(g|\bm{x},\bm{P}_{\hat{t}}) \cdot p(y|x, \bm{P}_{\hat{t}}) \cdot \mathbb{I}_{y \in Y^g},
\end{equation}
where $\mathbb{I}_{y \in Y^g}=1$ if $y\in Y^g$, else 0. The value of $p(g|\bm{x}, \bm{P}_{\hat{t}})$ is calculated based on the "energy" of $\bm{x}$ w.r.t group $g$, in relation to other group $g' \neq g$:
% \vspace{-3mm}
\begin{align}
p(g|\bm{x},\bm{P}_{\hat{t}}) = \frac{\exp \{ E(\bm{x}, g) \}}{\sum_{g' \in \mathcal{G}} \exp \{ E\left(\bm{x}, g' \right)\}}.
\label{test:predictG}
\end{align}
In Eq. (\ref{test:predictG}), $E\left(\bm{x}, g\right)$ indicates the "energy" of $\bm{x}$ w.r.t leaf group $g\in \mathcal{G}$. Remind that for each class $c$, we maintain a GMM of $K$ mixtures $\{\mathcal{N}(\boldsymbol{\mu}_{c,i}, \Sigma_{c,i})\}_{i=1}^K$. Based on the prototypes for a class, we can define the distance from $\bm{x}$ to a class $c$ as $d(\vx, c)= \min_{1\leq i \leq K} cosine\_distance(\vz_x, \boldsymbol{\mu}_{c,i})$. Limiting to the group $g$, we define $\hat{y}_\vx^g = \argmin_{c \in Y^g} d(\vx, c)$ (i.e., $Y^g$ is the set of all classes in $g$). We define the energy of interest as
\begin{align}
    % E(\bm{x}, g) &= d_{closest}(\bm{x}, \hat{y}_{\bm{x}}^g) - \xi \sum_{c\in Y^g} \gamma_{c,\hat{y}_x^g} d_{M}(\vx, D_c) \\ 
E(\bm{x}, g)=- d(\vx, \hat{y}_x^g) - \xi \sum_{c\in Y^g} \gamma_{c,\hat{y}_x^g} \sum_{i=1}^{K} \sqrt{(\bm{z_x}-\mu_{c,i})^T\Sigma^{-1}_{c,i}(\bm{z_x}-\mu_{c,i})} 
\end{align}
where the first terms is the cosine similarity between $\bm{z_x}$ and the closest class prototype within group $g$ and $\gamma_{c,\hat{y}_x^g}$ is the value obtained from \textit{the weight matrix} $\Gamma$ (Section \ref{ot_tricky}) - indicating the correlation between class $c$. This approach exploits the correlation between $\vx$ and $g$ while reducing the disadvantage of large groups with many classes, whereby the distances of classes that are less related to $y$ will have less weight and vice versa. Finally, $\xi$ is the hyperparameter, which controls the amount of information referenced from the group.

By this strategy, features $\bm{z_x}$ will have an additional point of view to determine which class that $\bm{x}$ is more likely to belong to, especially for $\bm{z_x}$ located at the boundary between leaf groups—such as between the group of "Plants" and the group of "Four-legged animals". This is similar to how having more prior knowledge improves posterior probability in Bayes' rule and how humans with more in-depth knowledge in different fields have greater experience in solving problems.

% This provides extra reference data as a useful prior, enhancing the posterior in the model's judgment


==> arvix/A_sec/4-exp.tex <==
\subsection{Experimental setup}

\textbf{Datasets.} We examine widely used CIL benchmarks, including Split CIFAR-100, Split ImageNet-R, 5-Datasets, and Split CUB-200 (please refer Appendix \ref{Datasets} for more details).


\textbf{Baselines.} We compare our method with notable CL methods exploiting prompt-based approach for pre-trained models, including the methods using shared prompts for all tasks: L2P \citep{wang2022learning_l2p}, DualPrompt \citep{wang2022dualprompt}, OVOR \citep{DBLP:conf/iclr/HuangCH24}; and the methods dedicates a distinct prompt set for each task like: S-Prompt++ \citep{wang2022sprompts}, CODA-Prompt \citep{smith2022coda}, HiDe-Prompt \citep{wang2023hierarchical}, CPP \citep{li2024steering}. 

\textbf{Metrics.} We use two main metrics, including the Final Average Accuracy (FAA), denoting the average accuracy after learning the last task, and the Final Forgetting Measure (FFM) showing the forgetting of all tasks after learning the sequence of tasks (see Appendices \ref{baselines} \& \ref{metrics}). 

The implementation is described in detail in Appendix \ref{Implementation}.

% For convenience, we denote two variations of our method without the self-improvement process: (i) \textit{\textbf{BoostCL-s}} is the version that uses the task-adaptive backbone with a single classifier for the CP-based backbone, while (ii) \textit{\textbf{BoostCL-m}} is the version that utilizes our proposed ensemble classifier with the boosting strategy for multiple views.

% \vspace{-5mm}

\subsection{Experimental result}

\paragraph{Our approach achieves superior results compared to baselines.} Table \ref{table:main_results} presents the overall performance comparison between our proposed method and all the baselines. The key observation is that our method is the strongest one with the gap between our method and the runner-up method is about 2\% in terms of FAA on all considered datasets. Additionally, the results show that our method avoids forgetting better than all baselines, notably reducing forgetting by more than 2\% on the Split-CIFAR100 dataset compared to the strongest one.


% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table*}[!ht]
	\centering
    % \vspace{-0.3cm}
    \caption{Overall performance comparison. We provide FAA and FFM of all methods, with standard deviation taken over at least 3 runs of different random seeds. The results corresponding to the best FAA among baselines are underlined.}.
    \vspace{-0.3cm}
    %\cite{smith2022coda} uses self-supervised pre-training on ImageNet-21K with supervised fine-tuning on ImageNet-1K, and different data splits for ImageNet-R. Here we reproduce its results with the same settings.
    
      %\vspace{-0.1cm}
	\smallskip
      \renewcommand\arraystretch{2.0}
    \small{
	\resizebox{1.0\textwidth}{!}{ 
	\begin{tabular}{l cc cc cc cc}
	 \hline
        % \multirow{2}{*}{PTM} & \multirow{2}{*}{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, Method} & \multicolumn{3}{c|}{Split CIFAR-100} & \multicolumn{3}{c|}{Split ImageNet-R} & \multicolumn{3}{c|}{5-Datasets} & \multicolumn{3}{c}{Split CUB-200} \\
        % & & \textbf{FAA} ($\uparrow$) & CAA ($\uparrow$) & FFM ($\downarrow$) & \textbf{FAA} ($\uparrow$) & CAA ($\uparrow$) & FFM ($\downarrow$) & \textbf{FAA} ($\uparrow$) & CAA ($\uparrow$) & FFM ($\downarrow$) & \textbf{FAA} ($\uparrow$) & CAA ($\uparrow$) & FFM ($\downarrow$)\\
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{Split CIFAR-100} & \multicolumn{2}{c}{Split ImageNet-R} & \multicolumn{2}{c}{5-Datasets} & \multicolumn{2}{c}{Split CUB-200} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        & \textbf{FAA} ($\uparrow$)  & FFM ($\downarrow$) & \textbf{FAA} ($\uparrow$) &  FFM ($\downarrow$) & \textbf{FAA} ($\uparrow$)  & FFM ($\downarrow$) & \textbf{FAA} ($\uparrow$) &  FFM ($\downarrow$)\\
        \hline
    %    \multirow{6}*{\tabincell{c}{Sup-21K}} 
       L2P &83.06 \small{$\pm 0.17$} &6.58 \small{$\pm 0.40$} &63.65 \small{$\pm 0.12$} &7.51 \small{$\pm 0.17$} & 81.84 \small{$\pm 0.95$}  & 4.58 \small{$\pm 0.53$} & 74.52 \small{$\pm 0.92$} & 11.25 \small{$\pm 0.23$} \\ 
       
       DualPrompt &86.60 \small{$\pm 0.19$} &4.45 \small{$\pm 0.16$} &68.79 \small{$\pm 0.31$} &4.49 \small{$\pm 0.14$} &77.91\small{$\pm 0.45$} & 13.17 \small{$\pm 0.71$} & 82.05\small{$\pm 0.95$} & 3.56 \small{$\pm 0.53$} \\ 

       OVOR & 86.68 \small{$\pm 0.22$} & 5.25 \small{$\pm 0.12$} & \underline{75.61 \small{$\pm 0.82$}}& 5.77 \small{$\pm 0.12$} & 82.34 \small{$\pm 0.48$} & 4.83 \small{$\pm 0.35$} & 78.12 \small{$\pm 0.0.65$} & 8.13 \small{$\pm 0.52$} \\ 
       \hline 
       S-Prompt++ &88.81 \small{$\pm 0.18$} &3.87 \small{$\pm 0.05$} & 69.68 \small{$\pm 0.12$} &3.29 \small{$\pm 0.05$} &86.19\small{$\pm 0.65$} & 4.67 \small{$\pm 0.72$} & 83.12 \small{$\pm 0.54$} & 2.72 \small{$\pm 0.64$} \\
       
       CODA-P &86.94 \small{$\pm 0.63$} &4.04 \small{$\pm 0.18$} & 70.03 \small{$\pm 0.47$}& 5.17 \small{$\pm 0.22$} & 64.20 \small{$\pm 0.53$} & 17.22 \small{$\pm 0.55$} & 74.34 \small{$\pm 0.68$}  & 12.05 \small{$\pm 0.41$} \\

       CPP &91.12 \small{$\pm 0.12$} & 3.33 \small{$\pm 0.18$} & 74.88 \small{$\pm 0.07$} & 4.08 \small{$\pm 0.03$} & 92.92 \small{$\pm 0.17$} & \underline{0.23 \small{$\pm0.07$}} & 82.35 \small{$\pm0.23$} & 3.24 \small{$\pm0.32$} \\
       
       HiDe-Prompt  &\underline{{92.61} \small{$\pm 0.28$}} &\underline{{1.52} \small{$\pm 0.10$}}  &{75.06 \small{$\pm 0.12$}} & \underline{4.05 \small{$\pm 0.19$}} & \underline{93.92 \small{$\pm 0.33$}}  & 0.31 \small{$\pm 0.12$}  & \underline{86.62 \small{$\pm 0.35$}} & \underline{2.55 \small{$\pm0.15$}} \\
       
       \midrule
    
        % Ours (train only) & \textbf{93.94} \small{$\pm 0.22$} &  \textbf{1.56} \small{$\pm 0.18$} & \textbf{76.41} \small{$\pm 0.12$} & \underline{3.12 \small{$\pm 0.25$}} & \textbf{95.02} \small{$\pm 0.18$} & \underline{0.25 \small{$\pm 0.16$}} & \textbf{87.93} \small{$\pm 0.18$} & \underline{2.52 \small{$\pm 0.22$}} \\

        Ours (TCL) & \textbf{94.52} \small{$\pm 0.22$} &  \textbf{1.02 \small{$\pm 0.18$}} & \textbf{77.01} \small{$\pm 0.12$} & \textbf{4.03 \small{$\pm 0.25$}} & \textbf{95.35} \small{$\pm 0.18$} & \textbf{0.20 \small{$\pm 0.16$}} & \textbf{88.33} \small{$\pm 0.18$} & \textbf{1.98 \small{$\pm 0.22$}} \\
       
       \midrule
       
       % \hline
       
	\end{tabular}
	} }
	\label{table:main_results}
	\vspace{-0.3cm}
\end{table*}

\paragraph{Our training strategy improves model performance significantly.} 
Figure \ref{fig:ablate_train} reports the ablation studies demonstrating the effectiveness of our training strategy. Particularly, compared to training tasks independently using Cross Entropy loss $\mathcal{L}_{CE}$ like in DualP, L2P, and CODA-P, exploiting the relationships between data classes with the label-based hierarchical taxonomy and the WD-based cost matrix helps improve FAA by about 5\% to 10\% (Figure \ref{fig:ablate_LG}). Besides, when examining the role of exploiting additional prior information from pretrained backbones using the OT approach, we see that FAA is improved from 0.6\% to 0.8\% (Figure \ref{fig:ablateOT}). These results demonstrate the positive impact of this component, confirming the importance of exploiting correlations between class data during training. In both figures, the improvements on Split-CIFAR100 and 5-Datasets are the lowest, while it is more pronounced on Split-CUB-200. This may be because the groups of these two datasets (Split-CIFAR100 and 5-Datasets) have fewer overlapping classes, as the classes in each group likely have more recognizable features. Meanwhile, Split-CUB-200 is a dataset about birds, with images that can be difficult for human eyes to recognize, thus so our method performs better.

In addition, Figure \ref{fig:ablate_alphabeta} provides the experimental results on Split-CUB-200 dataset, when varying $\alpha$ and $\beta$, which control the intensification of impact on each leaf group of $\mathcal{L_G}$ during training. The data shows that with a large enough value of $\beta$, our HiT is not sensitive to $\alpha$ within its acceptable range. Conversely, if $\alpha$ is small, the quality of the model can change more significantly.

Furthermore, Figure \ref{fig:tnse} illustrates the effect of our method in improving model's representation learning on Split-CIFAR100. Specifically, the classes are better clustered, and the separation between them is more distinct. Especially, the classes 'oak tree,' 'willow tree,' and 'pine tree' are divided into clear clusters, rather than being mixed together as in the traditional training strategy, where tasks are trained independently.
\vspace{-3mm}
\begin{figure}[htbp]
    \centering
    % Subfigure 1
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/role_train.pdf} % Replace with your image file
        \caption{The role of $\mathcal{L_G}$}
        \label{fig:ablate_LG}
    \end{subfigure}
    \hfill
    % Subfigure 2
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/role_ot.pdf} % Replace with your image file
        \caption{The role of OT-based strategy}
        \label{fig:ablateOT}
    \end{subfigure}
    \hfill
    % Subfigure 3
    \begin{subfigure}[b]{0.325\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/alpha_beta.pdf} % Replace with your image file
        \vspace{0.36mm}
        \caption{Varying the value of $\alpha, \beta$}
        \label{fig:ablate_alphabeta}
    \end{subfigure}
    \caption{Ablation study about our training strategy.}
    \label{fig:ablate_train}
\end{figure}
\vspace{-3mm}
\paragraph{Our testing strategy has positive effects for final prediction} Table \ref{table:testing} illustrates the improvement of FAA on all considered datasets when applying our testing strategy, from about 0.4\% to 0.6\%. 
This proves the approach to be effective, as the information from each cluster provides a reference channel that helps determine the identity of the classes, offering a good suggestion for future studies.

\begin{table}[ht]
    % \vspace{-0.5cm}
    \centering
    \caption{Effectiveness of our testing strategy.} 
     % \vspace{-0.2cm}
	\smallskip
      \renewcommand\arraystretch{1.5}
      % \setlength\tabcolsep{2.5pt}
    \small{
	\resizebox{0.8 \textwidth}{!}{ 
        \centering
	\begin{tabular}{lcccc}
	 \hline
      Dataset & {Split CIFAR-100} & {Split Imagenet-R} & {5-Datasets} & {Split CUB-200} \\
        \hline
        Normal testing & 93.94  & 76.41 & 95.02 & 87.93 \\
        Our testing strategy & \textbf{94.52} & \textbf{77.01} & \textbf{95.35} & \textbf{88.33} \\
       \hline
	\end{tabular}
	} 
}
	\label{table:testing}
	% \vspace{-0.56cm}
\end{table}





% \begin{table}[ht]
%     % \vspace{-0.5cm}
%     \centering
%     \caption{Comparison when using different pretrained backbones} 
%      % \vspace{-0.2cm}
% 	\smallskip
%       \renewcommand\arraystretch{1.5}
%       % \setlength\tabcolsep{2.5pt}
%     \small{
% 	\resizebox{0.5 \textwidth}{!}{ 
%         \centering
% 	\begin{tabular}{lcccc}
% 	 \hline
%       \multirow{2}{*}{Pretrained backbone} & \multicolumn{2}{c}{Split CIFAR-100} & \multicolumn{2}{c}{Split Imagenet-R} \\
%       \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
%         & HiT & HiDE & HiT & HiDE \\
%         \hline
%        Sup-21K & \textbf{93.94} \textcolor{blue}{\small{$(\uparrow 1.33)$}} & 92.61 & \textbf{76.41} & 75.06\\
%        iBOT-21K & \textbf{94.01} & 93.02 & \textbf{72.12} & 70.83\\
%        iBOT-1K & \textbf{94.27} & 93.48 & \textbf{72.80} & 71.33\\
%        DINO-1K & \textbf{94.12} & 93.51 & \textbf{69.25} & 68.11\\ 
%        MoCo-1K & \textbf{92.32} & 91.57 & \textbf{64.23} & 63.77 \\
%        \hline
% 	\end{tabular}
% 	} 
% }
% 	\label{table:backbone}
% 	% \vspace{-0.56cm}
% \end{table}







==> arvix/A_sec/5-conclusion.tex <==
In this work, we demonstrate the importance of organizing and exploiting data meaningfully rather than lumping it together for training. Organizing data into a tree-like taxonomy based on label information gives us a new perspective on the data. Particularly, we can divide them into small groups containing the classes that are likely to confuse models. This approach encourages the model to focus and build deeper knowledge for each group, thereby reducing forgetting and motivating more effective learning in subsequent tasks. Additionally, we introduce a new perspective by leveraging the initial behavior of pretrained models, providing an additional information channel to further improve performance. Besides, our testing strategy has shown positive effects by exploiting group knowledge during inference. Finally, experimental results demonstrate the effectiveness of these components and our superiority over state-of-the-art baselines.

\paragraph{Limitation discussion.}Despite this novel perspective, the quality of the hierarchical taxonomy depends on the quality of expert knowledge. For example, if similar image classes are not assigned to the same leaf group in this label-based taxonomy, the constraint we put on each such group may not perform as expected. Furthermore, although the testing strategy shows positive results, to exploit group knowledge more efficiently, it is necessary to further investigate to understand the characteristics and hidden structure of data.





==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

